Poincar\'e's Odds

This paper is devoted to Poincar\'e's work in probability. Though the subject does not represent a large part of the mathematician's achievements, it provides significant insight into the evolution of Poincar\'e's thought on several important matters such as the changes in physics implied by statistical mechan- ics and molecular theories. After having drawn the general historical context of this evolution, I focus on several important steps in Poincar\'e's texts dealing with probability theory, and eventually consider how his legacy was developed by the next generation.

==> bourbaphydefs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin of definition file AHPEFS.TEX                      %
% (c) Stephan Ammann, for Birkhaeuser, Dec 1999            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AHPDEFS.tex -- is red in by each header file             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\font\fxtit=cmssbx10 % For the new logo

\newcount\fpage\newcount\npage\newcount\lpage
\fpage=\fipage\npage=\nrpage
\lpage=\fpage\advance\lpage by\npage\advance\lpage by-1

\def\xrule{\vrule width2.25pt}
\def\yrule{\hrule height.5pt}
\def\yrulefill{\leaders\yrule\hfill}
\def\strutx{\vrule height8.5pt width0pt depth0pt}
\def\struty{\vrule depth3.5pt width0pt}
\def\strutz{\vrule height10.2pt width0pt}

\def\boxl{\vbox{\halign{##\hfil\cr
{\sc Poincar\'e}, 1912-2012, S{\'e}minaire Poincar{\'e} \volnr\  (\centnr\yearnr)
\the\fpage\ -- \the\lpage\cr
%\struty \copyright\ Birkh{\"a}user Verlag, Basel,
%\centnr\yearnr\cr
%1424-0637/\yearnr/\issuenr0\fipage-\the\npage\ \ %
%\$\,1.50$+$0.20/0\cr
}}}


\def\boxr{\vbox{\offinterlineskip
\halign{##\hfil\hskip1mm&##\hfil\cr
\noalign{\vskip.8mm}
\multispan2{\yrulefill}\cr
\xrule\strutz\struty
&\fxtit S{\'e}minaire Poincar{\'e}\cr
%\xrule\strutx&%
%\vbox to0pt{%
%\vbox to0pt{\vss\hbox{\fxtit and Applications NoDEA}}\vss}\cr
}}}

\def\titlebox{\vbox to0pt{\hsize=150mm\footnotesize\vss
\hbox to\hsize{\boxl\hfil\boxr}}}


\def\ps@myheadings{
\let\@mkboth\markboth
\def\@oddhead{\footnotesize {\sc Poincar\'e}, 1912-2012, \rm Vol. \volnr,  \centnr\yearnr
\hspace{6mm}\titletxt\hfil\thepage}%
\def\@oddfoot{} % % centered page number
\def\@evenhead{\footnotesize \thepage \hfil
\authortxt\hspace{6mm}S{\'e}minaire Poincar{\'e}}%
\def\@evenfoot{}%       % centered page number
}

\def\ps@plain{
\let\@mkboth\markboth
\def\@oddhead{%
\titlebox}%
\def\@oddfoot{}%      % centered page number
\def\@evenhead{}%
\def\@evenfoot{}%     % centered page number
}

\ps@myheadings              % 'myheading' page style
\pagenumbering{arabic}      % Arabic page numbers
\onecolumn                  % Single-column.

\setcounter{page}{\fpage}

\textwidth=150mm
\textheight=230mm
\parindent=8mm
\evensidemargin=0pt
\oddsidemargin=0pt
\topmargin=0pt
\frenchspacing

\newcommand{\pdpg}{\postdisplaypenalty=-2000}
%% Used to force a page-break after a displayed equation

\let\dst=\displaystyle
\let\scr=\scriptstyle

\def\bfdefault{b}

\def\Rec{Received\ }
\def\Rev{Revised\ }

\endinput

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% End of AHPDEFS.TEX                                       %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% End of definition file

%%% Local Variables: 
%%% mode: plain-tex
%%% TeX-master: t
%%% TeX-master: t
%%% TeX-master: t
%%% End: 

